The connectivity degree controls the difficulty of RBN reservoir design

Reservoir Computing (RC) is a paradigm in artificial intelligence where a recurrent neural network (RNN) is used to process temporal data, leveraging the inherent dynamical properties of the reservoir to perform complex computations. In the realm of RC, the excitatory-inhibitory balance b has been shown to be pivotal for driving the dynamics and performance of Echo State Networks (ESN) and, more recently, Random Boolean Network (RBN). However, the relationship between b and other parameters of the network is still poorly understood. This article explores how the interplay of the balance b, the connectivity degree K (i.e., the number of synapses per neuron) and the size of the network (i.e., the number of neurons N) influences the dynamics and performance (memory and prediction) of an RBN reservoir. Our findings reveal that K and b are strongly tied in optimal reservoirs. Reservoirs with high K have two optimal balances, one for globally inhibitory networks (b<0), and the other one for excitatory networks (b>0). Both show asymmetric performances about a zero balance. In contrast, for moderate K, the optimal value being K=4, best reservoirs are obtained when excitation and inhibition almost, but not exactly, balance each other. For almost all K, the influence of the size is such that increasing N leads to better performance, even with large values of N. Our investigation provides clear directions to generate optimal reservoirs or reservoirs with constraints on size or connectivity.

==> performances.tex <==
\section{What drives performances} \label{p3:main}

In this section, we examine whether there is a relationship between reservoir dynamics in the absence of input, as explored in the previous section, and its ability to perform two demanding tasks: memory and prediction. This is done in two steps:
\begin{itemize}
    \item \textbf{Connectivity, attractor, and performance:} In section \ref{p3:performance}, we analyze the performance obtained separately in each task, depending on the control parameter, for each dominant attractor category. We show that the key factor driving performance is the excitatory/inhibitory balance.
    \item \textbf{Attractor and cross-task performance:} In section \ref{p3:cross}, we analyze all reservoir performances independently of the control parameter. For each reservoir, we study the relationship between the performance obtained in each task and their dominant attractor. This allows us to deduce how to generate a reservoir for the best general purpose.
\end{itemize}

From now on, and for ease of notation, a reservoir with a dominant attractor obtained during free evolution (defined in previous section \ref{p2:dominant}) will be referred to as either: a \textit{extinguished}, \textit{fix}, \textit{cyclic}, or \textit{irregular} reservoir (e.g., an \textit{extinguished reservoir} refers to a reservoir with an extinguished dominant attractor).

\subsection{Performance in memory and prediction tasks} \label{p3:performance}

Close to the critical points, we obtained various dominant attractors for a single value of $\sigma^\star$. This raises an important question regarding the relationship between the dominant attractor of a reservoir and its performance. Specifically, it is worth investigating whether the dominant attractor influences the reservoir's performance. If this is the case, grouping attractor categories by discrete performance levels may be possible based on a single value of $\sigma^\star$.

\subsubsection{Methodolody:} We evaluate the performance of the networks to execute two fundamental tasks: \textit{memory} and \textit{prediction}. Each reservoir receives an input $u(t)$, and the readout target is $T(t)=u(t+\delta)$, equal to the input shifted in time by  $\delta$ time steps. $\delta<0$ corresponds to a memory task, and $\delta>0$ to a prediction task. For each value of $\sigma^{\star}$, we use 100 reservoirs, and each reservoir is run five times, with a different random tossing of the input weight matrix (more detail on the training procedure in \textbf{S}\ref{suppm:training}). 

\begin{figure*}
\centering
    \includegraphics[scale=0.56]{images/panel3.jpg}
    \caption{Performances for two tasks: white noise memory (\textbf{C}, \textbf{E}); and Mackey-glass prediction (\textbf{D}, \textbf{F}). \textbf{A} and \textbf{D}: examples of signals for each task with their respective parameters. \textbf{A}: White noise memory task, which consists in remembering the input (\textcolor{darkgray}{gray}), to reproduce it in output (\textcolor{darkred}{dark red}) with a negative delay $\delta$ (shown example corresponds to $\delta=-6$). \textbf{B}: Mackey glass is controlled by the parameter $\tau$ (see methodology \ref{suppm:performance} for more details), ranging from periodic to chaotic. \textbf{C}, \textbf{D}, \textbf{E}, \textbf{F}: the average performance $Corr(y, T)$ between the output $y$ and target $T$, plotted over $|\sigma^\star|$, for each dominant attractor category: \textit{no-activity}, \textit{fix}, \textit{cyclic} or \textit{irregular}. For each value of $\sigma^\star$ we have $100$ reservoirs. The solid line then represents the average over reservoirs belonging to the same attractor category; individual reservoir performances are averaged over $5$ initial conditions. The shaded area represents one standard deviation. Higher correlations indicate better performance. The hatched gray area represents the critical regions, as defined in section \ref{p2:activity}. \textbf{C} and \textbf{D}: the performance in the white-noise memory task; three values of $\delta$ are tested: $-2$ ($\star$), $-6$ ($\bullet$), $-10$ ($\blacktriangledown$). \textbf{E} and \textbf{F}: the performance of Mackey-Glass prediction ($\delta=+10$); three values of $\tau$ are tested: $5$ ($\star$), $20$ ($\star$), $50$ ($\blacktriangledown$). \textbf{C} and \textbf{D}: Performance for $\sigma^{\star}<0$, with inside each plot a zoom on the critical region. \textbf{E} and \textbf{F}: performance for $\sigma^{\star}>0$.}
\label{fig:panel3}
\end{figure*}

The first task consists of memorizing a purely random signal (i.e., uncorrelated white noise), and since there is absolutely no correlation in the input, only memorization is involved. Fig.~\ref{fig:panel3}.\textbf{A} illustrates this task for one value of $\delta=-6$, with white noise as input $u$, and the target $T$. 

For the second task, we explore the ability of the reservoir to predict a time series, $\delta=10$ time steps in the future. The input is the well-known Mackey-Glass time series, as it is a common benchmark of this type of task (\cite{Hajnal2006}, \cite{Goudarzi2016a}, \cite{Canaday2018}, among others), notably testing the ability to infer  non-linear dynamics. The signal regularity is controlled by the parameter $\tau$, see Fig.~\ref{fig:panel3}.\textbf{B}, ranging from periodic with $\tau=5$, to chaotic for $\tau=28$ (more information on the experiments in \textbf{S}\ref{suppm:performance}).

\subsubsection{Analysis:}
The performance of a reservoir is measured by computing the correlation product $Corr(y,T)$ between the output $y$ and the target $T$. A perfect match corresponds to a correlation of one, while a random output gives a zero correlation. An individual reservoir performance score is then obtained by averaging over the initial conditions. Each individual reservoir is associated with its dominant attractor, and the statistics of the performance of reservoirs are performed separately for each attractor.

\subsubsection{Results:} 
The average performance is plotted as a function of $|\sigma^{\star}|$ in Fig.~\ref{fig:panel3}\textbf{C,E} for the memory task and in Fig.~\ref{fig:panel3}\textbf{D,F} for the prediction task. The left column (\textbf{C} and \textbf{D}) corresponds to $\sigma^\star>0$, and the right column (\textbf{E} and \textbf{F}) to $\sigma<0$. The colour of the lines corresponds to the attractor. 

For $\sigma^\star < 0$ (Fig.~\ref{fig:panel3}.\textbf{C} and \textbf{D}), performance increases over a very wide range of $\sigma^\star$, both for memory and prediction. This range includes the critical region (gray hatched area) but is vastly broader. Thus, being within the critical region is absolutely not mandatory to perform well. A shaded area in Figs.~\ref{fig:panel3} indicates the spreading of the results. There is none in plots \textbf{C} and \textbf{D}, meaning that all reservoirs perform exactly the same for a given $\sigma^\star$. Moreover, as $\sigma^\star$ is increased through the critical region, the dominant attractors change (see zooms in plot \textbf{C} and \textbf{D}), but surprisingly, there is no discontinuity in the performance. Indeed, even though the four attractor categories are present inside the gray area, their respective performance all align. This strongly suggests that the dynamics of the reservoir, as measured in the absence of input, is irrelevant for the performance. Only the value of $\sigma^\star$ matters. In both tasks, the average performance decreases monotonically with increasing difficulty via $\tau$ and $\delta$. In the memory task, we register a dip in performance close to the critical point. This goes against the common assumption that the edge of chaos is optimal for memory \cite{Natschlager2005}. In the prediction task, the peak of performance roughly coincides with the critical region, except for the greater difficulty, where the peak is slightly on the left. 

The picture is very different for $\sigma^\star > 0$ (Figs.~\ref{fig:panel3}\textbf{E} and \textbf{F}). First, the region in which some level of performance is observed is comparable to the critical region observed in free-running reservoirs. Second, there is substantial variability in performance across different reservoirs, as indicated by the large shaded areas. Despite this variability, there is an overall dependence of performance on $\sigma^\star$. The average performance of distinct dominant attractor categories is much noisier. However, despite being more noisy, the average performance of the distinct attractor categories aligns again, so there is still no evidence that the attractor category has any significant impact on the reservoir's performance. We observe that performance decreases as the difficulty of the memorization task increases, but interestingly, this trend appears to be inverted in the prediction task.

Once again, the two signs of  $\sigma^\star$ give rise to different behaviour. In particular,  networks with $\sigma^\star > 0$ memorize better and are less reliable than those with $\sigma^\star < 0$ but have poorer prediction capability. Yet, in all cases, attractors do not seem to be correlated to performance, as the top performance can be found in any of the four attractor categories.

 
\subsubsection{Discussion:}
Our results somewhat challenge the common assumption that the edge of chaos is optimal for performance and suggest that this is true for reservoirs with a majority of excitation but not necessarily with a majority of inhibition. Reservoirs with negative $\sigma^\star$ exhibit very reliable performances with very low reservoir-to-reservoir variability over a range in  $\sigma^\star$ much broader than the critical region. Since reservoirs behave the same, in practice, it is sufficient to generate one, with $\sigma^\star$ at the left of the critical region. However, if the goal is optimal memorization, it is wiser to choose $\sigma\sim0.4$ in the critical region and try different reservoirs until finding a good one, which requires training and testing.

\subsection{Cross-task performance} \label{p3:cross}
Beyond studying the performance in memorization and prediction separately, as often done (\cite{Bertschinger2004c}, \cite{Busing2010}), here we aim at answering the following question: are the reservoirs intrinsically good or bad, or does it depend on the task? In other words, are there general-purpose reservoirs and specialized ones? 

\subsubsection{Analysis:}
We analyze the absolute value of the performance of all reservoirs independently of the control parameter. For each reservoir, we study its performance in the memory task as a function of its performance in the prediction tasks (see section \ref{p3:performance} \textit{methodology}). For this, we fixed values of $\delta$ (memory) and $\tau$ (prediction), and we chose three levels of difficulty: simple ($\tau=5$, $\delta=-2$), average ($\tau=20$, $\delta=-6$) and difficult ($\tau=28$, $\delta=-10$).

\begin{figure*}
\centering
    \includegraphics[scale=0.6]{images/panel4.jpg}
    \caption{The performance of all reservoirs in the prediction tasks (Mackey-Glass) as a function of their performance in the memory tasks (white-noise), for $\sigma^\star<0$ (\textbf{A}, \textbf{B}, \textbf{C}) and $\sigma^\star>0$ (\textbf{D}, \textbf{E}, \textbf{F}). Reservoirs are again classified according to their dominant attractor (see supplementary material S\ref{suppm:stat_dominant}). Each dot represents an individual reservoir performance averaged over $5$ initial conditions. In all plots, dots with black edges display reservoirs taken at the critical regimes. We chose three different pairs of values for the parameters of the tasks, $\tau$ and $\delta$, each representing a different difficulty level: 1. Simple (\textbf{A} and \textbf{D}) the lowest difficulty in both tasks, $\tau=5$ and  $\delta=-2$; 2. Average (\textbf{B} and \textbf{E}) average difficulty for intermediary values of $\tau=20$ and $\delta=-6$; 3. Difficult (\textbf{C} and \textbf{F}) difficult task for higher values of $\tau=28$ and $\delta=-10$.}
\label{fig:panel4}
\end{figure*}

\subsubsection{Results:}
Fig.~\ref{fig:panel4} displays the performance of reservoirs as coloured dots. As in the previous section, each colour corresponds to the dominant attractor of the reservoir. The vertical axis represents the performance in the prediction task (Mackey-Glass), and the horizontal axis that of the memory task (white noise). The columns correspond to the sign of $\sigma^\star$, negative on the left, positive on the right. The rows correspond to the degree of difficulty, from simple (top) to difficult (bottom). 

For $\sigma^{\star}<0$ (left column), there is an apparent relationship in performance between the two tasks. The degree of difficulty roughly acts as a scaling factor on the curves, but the correlation is always clear. The reservoirs which are good at predicting do memorize well as well. There is, however, a reentrant region of irregular reservoirs (red) which are the best at memorizing but are not optimal for predicting, in particular for the intermediate degree of difficulty (see the red loop on Fig.~\ref{fig:panel4}\textbf{B}). This point corresponds to the maximum on the right of the dip observed in Fig~\ref{fig:panel3}\textbf{C}. Interestingly, in all difficulties, reservoirs at the critical point (encircled dots) create a narrow area with a good overall performance. This picture refines our previous analysis of the impact of attractors on performance, as it seems that extinguished reservoirs can perform slightly better at memory than the others, and the same for the irregular reservoirs at prediction. Nonetheless, the difference between attractors is rather small, and it could be argued that it is insignificant.


The picture is very different for $\sigma^\star>0$ (right column). Performances are distributed as clouds of points. In Fig.~\ref{fig:panel3}, we observe a large reservoir variability in both tasks. Some reservoirs are suitable for one task and bad for the other one. For intermediate and difficult tasks, some reservoirs outperform the best ones with $\sigma^\star<0$ in both memorization and prediction. Reservoirs at the critical point are found on the right of the plots, i.e. they promise good memorization but are nonetheless widely spread, especially in prediction (vertical axis). Overall, the distinct attractors occupy the space in overlapping and indistinguishable clouds; this confirms the previous analysis that attractors do not play a role in performance.

\subsubsection{Discussion:}
Correlations in performances are very different for both signs of $\sigma^\star$. Choosing a reservoir with $\sigma^\star\sim-0.66$ ensures a good, general-purpose reservoir but with suboptimal performance. In contrast, going into the positive side of $\sigma^\star$ may lead to the best reservoirs in a given task or even better general purpose reservoirs, but this comes at a price: those gems cannot be found by the statistical analysis we have performed on their free running activity.


